Model Based Residual Policy Learning with Applications to Antenna Control

Non-differentiable controllers and rule-based policies are widely used for controlling real systems such as telecommunication networks and robots. Specifically, parameters of mobile network base station antennas can be dynamically configured by these policies to improve users coverage and quality of service. Motivated by the antenna tilt control problem, we introduce Model-Based Residual Policy Learning (MBRPL), a practical reinforcement learning (RL) method. MBRPL enhances existing policies through a model-based approach, leading to improved sample efficiency and a decreased number of interactions with the actual environment when compared to off-the-shelf RL methods.To the best of our knowledge, this is the first paper that examines a model-based approach for antenna control. Experimental results reveal that our method delivers strong initial performance while improving sample efficiency over previous RL methods, which is one step towards deploying these algorithms in real networks.

==> algorithms/mbrpl.tex <==
\todo[inline]{We can add more details in the pseudo code, including the multi-update trick, and mention in the description that existing MBPO implementations did not work well on this problem.}
\todo[inline]{Comment: Did we try MBPO in the antenna env?}
\begin{algorithm}[t]
\caption{Model-Based Residual Policy Learning (MBRPL)}
\begin{algorithmic}[1]\label{alg:mbrpl}
    \REQUIRE Baseline policy $\pi_b$, parameters of the correction term $\phi=(\mu,\sigma)$
    \smallskip
    \STATE  Initialize transition model $p_{\theta}$, and initialize  critic $Q_{\psi}$ parametrized by $\psi$. 
    \STATE  Initialize replay buffer $\mathcal{B}$
    \FOR{epoch $=1,\dots,N$}
        \STATE Sample experiences from the true environment using $\pi_{\phi}^b$ and add them to $\mathcal{B}$
        \STATE Train $p_\theta$ on $\mathcal{B}$ using maximum-likelihood
        \STATE Use $(p_\theta, r, \pi_\phi^b)$ to generate trajectories and train $(\pi_\phi^b,Q_\psi)$ using off-policy actor critic methods
    % \FOR{each episode}
    %     \FOR{each time step}
    %         \STATE Sample action $a \sim \mathcal{N}( \mu_b(s) + \mu_{\phi}(s), \sigma_b(s) + \sigma_{\phi}(s)) $
    %         \STATE  Take action  environment step, add data to $\mathcal{B}$
    %         % \BlankLine
    %         \STATE  Train $p_{\theta}$ on data from buffer 
    %         % \BlankLine
    %         \STATE  Use $p_{\theta}$, $r$, $\pi$ to predict future states and rewards 
    %         \STATE  Train $f_{\phi}$ and $Q_{\psi}$ on real and predicted data 
    %     \ENDFOR
    % \ENDFOR
    \ENDFOR
    \end{algorithmic}
\end{algorithm}

